The Maven Dependency Graph: a Temporal Graph-based Representation of Maven Central

The Maven Central Repository provides an extraordinary source of data to understand complex architecture and evolution phenomena among Java applications. As of September 6, 2018, this repository includes 2.8M artifacts (compiled piece of code implemented in a JVM-based language), each of which is characterized with metadata such as exact version, date of upload and list of dependencies towards other artifacts. Today, one who wants to analyze the complete ecosystem of Maven artifacts and their dependencies faces two key challenges: (i) this is a huge data set; and (ii) dependency relationships among artifacts are not modeled explicitly and cannot be queried. In this paper, we present the Maven Dependency Graph. This open source data set provides two contributions: a snapshot of the whole Maven Central taken on September 6, 2018, stored in a graph database in which we explicitly model all dependencies; an open source infrastructure to query this huge dataset.

==> biblio.tex <==
%% LaTeX2e file `biblio'
%% generated by the `filecontents' environment
%% from source `main' on 2019/01/16.
%%
@inproceedings{raemaekers12,
  title={Measuring software library stability through historical version analysis},
  author={Raemaekers, Steven and van Deursen, Arie and Visser, Joost},
  booktitle={Software Maintenance (ICSM), 2012 28th IEEE International Conference on},
  pages={378--387},
  year={2012},
  organization={IEEE}
}

@inproceedings{Mitropoulos:2014:BCM:2597073.2597123,
 author = {Mitropoulos, Dimitris and Karakoidas, Vassilios and Louridas, Panos and Gousios, Georgios and Spinellis, Diomidis},
 title = {The Bug Catalog of the Maven Ecosystem},
 booktitle = {Proceedings of the 11th Working Conference on Mining Software Repositories},
 series = {MSR 2014},
 year = {2014},
 isbn = {978-1-4503-2863-0},
 location = {Hyderabad, India},
 pages = {372--375},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/2597073.2597123},
 doi = {10.1145/2597073.2597123},
 acmid = {2597123},
 publisher = {ACM},
 address = {New York, NY, USA},
}


@article{sourcerer,
title = "Sourcerer: An infrastructure for large-scale collection and analysis of open-source code",
journal = "Science of Computer Programming",
volume = "79",
pages = "241 - 259",
year = "2014",
note = "Experimental Software and Toolkits (EST 4): A special issue of the Workshop on Academic Software Development Tools and Techniques (WASDeTT-3 2010)",
issn = "0167-6423",
doi = "https://doi.org/10.1016/j.scico.2012.04.008",
url = "http://www.sciencedirect.com/science/article/pii/S016764231200072X",
author = "Sushil Bajracharya and Joel Ossher and Cristina Lopes",
}
@INPROCEEDINGS{Raemaekers13,
author={S. Raemaekers and A. van Deursen and J. Visser},
booktitle={2013 10th Working Conference on Mining Software Repositories (MSR)},
title={The Maven repository dataset of metrics, changes, and dependencies},
year={2013},
volume={},
number={},
pages={221-224},
doi={10.1109/MSR.2013.6624031},
ISSN={2160-1852},
month={May},}

@INPROCEEDINGS{Sajnani14,
author={H. Sajnani and V. Saini and J. Ossher and C. V. Lopes},
booktitle={2014 IEEE International Conference on Software Maintenance and Evolution},
title={Is Popularity a Measure of Quality? An Analysis of Maven Components},
year={2014},
pages={231-240},
doi={10.1109/ICSME.2014.45},
ISSN={1063-6773},
month={Sept},}

@article{mao2017survey,
  title={A survey of the use of crowdsourcing in software engineering},
  author={Mao, Ke and Capra, Licia and Harman, Mark and Jia, Yue},
  journal={Journal of Systems and Software},
  volume={126},
  pages={57--84},
  year={2017},
  publisher={Elsevier}
}

@INPROCEEDINGS{Kikas17,
author={R. Kikas and G. Gousios and M. Dumas and D. Pfahl},
booktitle={2017 IEEE/ACM 14th International Conference on Mining Software Repositories (MSR)},
title={Structure and Evolution of Package Dependency Networks},
year={2017},
pages={102-112},
month={May},}

@INPROCEEDINGS{pashchenko18,
author={Ivan Pashchenko and Henrik Plate and Serena Elisa Ponta and Antonino Sabetta and Fabio Massacci},
booktitle={Proceedings of the 12th International Symposium on Empirical Software Engineering and Measurement (ESEM)},
title={Vulnerable Open Source Dependencies: Counting Those That Matter},
year={2018},
month={Oct},
}

@inproceedings{de2014broad,
  title={A broad-coverage collection of portable NLP components for building shareable analysis pipelines},
  author={de Castilho, Richard Eckart and Gurevych, Iryna},
  booktitle={Proceedings of the Workshop on Open Infrastructures and Analysis Frameworks for HLT},
  pages={1--11},
  year={2014}
}

@inproceedings{Mileva09,
 author = {Mileva, Yana Momchilova and Dallmeier, Valentin and Burger, Martin and Zeller, Andreas},
 title = {Mining Trends of Library Usage},
 booktitle = {Proceedings of the Joint International and Annual ERCIM Workshops on Principles of Software Evolution (IWPSE) and Software Evolution (Evol) Workshops},
 series = {IWPSE-Evol '09},
 year = {2009},
 isbn = {978-1-60558-678-6},
 location = {Amsterdam, The Netherlands},
 pages = {57--62},
 numpages = {6},
 url = {http://doi.acm.org/10.1145/1595808.1595821},
 doi = {10.1145/1595808.1595821},
 acmid = {1595821},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {global usage trends, library versions usage, mining software archives},
}

@inproceedings{Mastrangelo15,
  author    = {Luis Mastrangelo and
               Luca Ponzanelli and
               Andrea Mocci and
               Michele Lanza and
               Matthias Hauswirth and
               Nathaniel Nystrom},
  title     = {Use at your own risk: the Java unsafe {API} in the wild},
  booktitle = {Proceedings of the 2015 {ACM} {SIGPLAN} International Conference on
               Object-Oriented Programming, Systems, Languages, and Applications,
               {OOPSLA} 2015, part of {SPLASH} 2015, Pittsburgh, PA, USA, October
               25-30, 2015},
  pages     = {695--710},
  year      = {2015},
  url       = {http://doi.acm.org/10.1145/2814270.2814313},
  doi       = {10.1145/2814270.2814313},
  timestamp = {Thu, 15 Jun 2017 21:39:51 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/oopsla/MastrangeloPMLH15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@InProceedings{Almeida11,
author="Almeida, H{\'e}lio
and Guedes, Dorgival
and Meira, Wagner
and Zaki, Mohammed J.",
editor="Gunopulos, Dimitrios
and Hofmann, Thomas
and Malerba, Donato
and Vazirgiannis, Michalis",
title="Is There a Best Quality Metric for Graph Clusters?",
booktitle="Machine Learning and Knowledge Discovery in Databases",
year="2011",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="44--59"
}

@inproceedings{mdd,
  author    = {Steven Raemaekers and
               Arie van Deursen and
               Joost Visser},
  title     = {The maven repository dataset of metrics, changes, and dependencies},
  booktitle = {Proceedings of the 10th Working Conference on Mining Software Repositories,
               {MSR} '13, San Francisco, CA, USA, May 18-19, 2013},
  pages     = {221--224},
  year      = {2013},
  url       = {https://doi.org/10.1109/MSR.2013.6624031},
  doi       = {10.1109/MSR.2013.6624031},
  timestamp = {Thu, 15 Jun 2017 21:40:38 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/msr/RaemaekersDV13},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
%% Dependency management references
@INPROCEEDINGS{Cox15,
author={J. Cox and E. Bouwers and M. v. Eekelen and J. Visser},
booktitle={2015 IEEE/ACM 37th IEEE International Conference on Software Engineering},
title={Measuring Dependency Freshness in Software Systems},
year={2015},
volume={2},
number={},
pages={109-118},
doi={10.1109/ICSE.2015.140},
ISSN={0270-5257},
month={May},}

@INPROCEEDINGS{Bavota13,
author={G. Bavota and G. Canfora and M. D. Penta and R. Oliveto and S. Panichella},
booktitle={2013 IEEE International Conference on Software Maintenance},
title={The Evolution of Project Inter-dependencies in a Software Ecosystem: The Case of Apache},
year={2013},
volume={},
number={},
pages={280-289},
keywords={Java;software engineering;software management;project inter-dependencies;software ecosystem;multiple software projects;Java subset;Apache ecosystem;API;Ecosystems;Software;Licenses;Libraries;Java;History;Data mining},
doi={10.1109/ICSM.2013.39},
ISSN={1063-6773},
month={Sept},}

@INPROCEEDINGS{Kula15,
author={R. G. Kula and D. M. German and T. Ishio and K. Inoue},
booktitle={2015 IEEE 22nd International Conference on Software Analysis, Evolution, and Reengineering (SANER)},
title={Trusting a library: A study of the latency to adopt the latest Maven release},
year={2015},
volume={},
number={},
pages={520-524},
doi={10.1109/SANER.2015.7081869},
ISSN={1534-5351},
month={March},}
%%dataset management

@InProceedings{Sajnani2014,
  author       = {Sajnani, Hitesh and Saini, Vaibhav and Ossher, Joel and Lopes, Cristina V},
  title        = {Is Popularity a Measure of Quality? An Analysis of Maven Components},
  booktitle    = {Software Maintenance and Evolution (ICSME), 2014 IEEE International Conference on},
  year         = {2014},
  pages        = {231--240},
  organization = {IEEE},
}

@InProceedings{Teyton2012,
  author    = {Teyton, Cedric and Falleri, Jean-Remy and Blanc, Xavier},
  title     = {Mining Library Migration Graphs},
  booktitle = {19th Working Conference on Reverse Engineering, WCRE 2012, Kingston, ON, Canada, October 15-18, 2012},
  year      = {2012},
  pages     = {289--298},
}

@InProceedings{Mileva2009,
  author       = {Mileva, Yana Momchilova and Dallmeier, Valentin and Burger, Martin and Zeller, Andreas},
  title        = {Mining trends of library usage},
  booktitle    = {Proceedings of the joint international and annual ERCIM workshops on Principles of software evolution (IWPSE) and software evolution (Evol) workshops},
  year         = {2009},
  pages        = {57--62},
  organization = {ACM}
}

@misc{rabbitmq,
 author = {{RabbitMQ}},
 title = {{RabbitMQ}},
 year = 2018,
 url = {\url{https://www.rabbitmq.com/}},
 note={[Online]. Available: \url{https://www.rabbitmq.com/}. [Accessed: 13- Nov- 2018].}
}

@misc{neo4j,
    author = {Neo4j Inc},
    title = {Neo4j},
    year = 2018,
 note={[Online]. Available: \url{https://www.neo4j.com/}. [Accessed: 13- Nov- 2018].}
}

@misc{aether,
    author = {Sonatype},
    title = {Aether},
    year = 2018,
 note={[Online]. Available: \url{https://wiki.eclipse.org/Aether/What_Is_Aether}. [Accessed: 13- Nov- 2018].}
}

@misc{cypher,
    author = {Neo4j Inc},
    title = {Cypher},
    year = 2018,
 note={[Online]. Available: \url{https://neo4j.com/developer/cypher-query-language/}. [Accessed: 13- Nov- 2018].}
}

@misc{cypher-usage,
    author = {OpenCypher},
    title = {OpenCypher Usages},
    year = 2018,
 note={[Online]. Available: \url{https://www.opencypher.org/projects}. [Accessed: 13- Nov- 2018].}
}

@misc{miner-proc,
    author = {Inria},
    title = {Maven-miner procedures},
    year = 2018,
 note={[Online]. Available: \url{ https://github.com/diverse-project/maven-miner/wiki/Maven-Miner-Procedures}. [Accessed: 13- Nov- 2018].}
}

@misc{maven-miner,
    author = {Inria},
    title = {Maven-miner},
    year = 2018,
 note={[Online]. Available: \url{ https://github.com/diverse-project/maven-miner/}. [Accessed: 13- Nov- 2018].}
}

@article{gai17modeling,
  title={Modeling Library Dependencies and Updates in Large Software Repository Universes},
  author={Gaikovina Kula, Raula and De Roover, Coen and German, Daniel M and Ishio, Takashi and Inoue, Katsuro},
  journal={arXiv preprint arXiv:1709.04626},
  year={2017}
}

@misc{sonatype-report,
    author = {Sonatype},
    title = {Sonatype Releases 2016 State of the Software Supply Chain Report},
    year = 2018,
 note={[Online]. Available: \url{https://www.sonatype.com/press-release-blog/ssc-press-release}. [Accessed: 13- Nov- 2018].}
}

@misc{maven-dep,
    author = {Inria},
    title = {Maven Dependency Graph. Version 06.09.2018-snapshot },
    doi = {10.5281/zenodo.1489120},
    year = 2018,
 note={[Online]. Available: \url{https://www.sonatype.com/press-release-blog/ssc-press-release}. [Accessed: 13- Nov- 2018].}
}


@inproceedings{kula2018generalized,
  title={A generalized model for visualizing library popularity, adoption, and diffusion within a software ecosystem},
  author={Kula, Raula Gaikovina and De Roover, Coen and German, Daniel M and Ishio, Takashi and Inoue, Katsuro},
  booktitle={2018 IEEE 25th International Conference on Software Analysis, Evolution and Reengineering (SANER)},
  pages={288--299},
  year={2018},
  organization={IEEE}
}


@misc{rogers2003diffusion,
  title={The diffusion of innovation 5th edition},
  author={Rogers, Everett M},
  year={2003},
  publisher={New York: Free Press}
}


==> utils.tex <==
\usepackage{soul}
\usepackage{tikz}

\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathmorphing}


\makeatletter

\newcommand{\defhighlighter}[3][]{%
  \tikzset{every highlighter/.style={color=#2, fill opacity=#3, #1}}%
}

\defhighlighter{yellow}{.5}

\newcommand{\highlight@DoHighlight}{
  \fill [ decoration = {random steps, amplitude=1pt, segment length=15pt}
        , outer sep = -15pt, inner sep = 0pt, decorate
        , every highlighter, this highlighter ]
        ($(begin highlight)+(0,8pt)$) rectangle ($(end highlight)+(0,-3pt)$) ;
}

\newcommand{\highlight@BeginHighlight}{
  \coordinate (begin highlight) at (0,0) ;
}

\newcommand{\highlight@EndHighlight}{
  \coordinate (end highlight) at (0,0) ;
}

\newdimen\highlight@previous
\newdimen\highlight@current

\DeclareRobustCommand*\highlight[1][]{%
  \tikzset{this highlighter/.style={#1}}%
  \SOUL@setup
  %
  \def\SOUL@preamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@BeginHighlight
      \highlight@EndHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@postamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@EndHighlight
      \highlight@DoHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@everyhyphen{%
    \discretionary{%
      \SOUL@setkern\SOUL@hyphkern
      \SOUL@sethyphenchar
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everyexhyphen##1{%
    \SOUL@setkern\SOUL@hyphkern
    \hbox{##1}%
    \discretionary{%
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everysyllable{%
    \begin{tikzpicture}[overlay, remember picture]
      \path let \p0 = (begin highlight), \p1 = (0,0) in \pgfextra
        \global\highlight@previous=\y0
        \global\highlight@current =\y1
      \endpgfextra (0,0) ;
      \ifdim\highlight@current < \highlight@previous
        \highlight@DoHighlight
        \highlight@BeginHighlight
      \fi
    \end{tikzpicture}%
    \the\SOUL@syllable
    \tikz[overlay, remember picture] \highlight@EndHighlight ;%
  }%
  \SOUL@
}

\makeatother

% Common abbrev. are set as commands to ensure proper spacing after the dot
\newcommand{\ie}{i.e.\@\xspace}
\newcommand{\aka}{a.k.a.\@\xspace}
\newcommand{\Aka}{A.k.a.\@\xspace}
\newcommand{\Ie}{I.e.\@\xspace}
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\Cf}{Cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
\newcommand{\Eg}{E.g.\@\xspace}
\newcommand{\etal}{et al.\@\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\Wrt}{W.r.t.\@\xspace}


\newcommand{\amine}[1]{\mynote{Amine}{#1}}
\newcommand{\benoit}[1]{\mynote{Benoit}{#1}}
\newcommand{\cesar}[1]{\mynote{Cesar}{#1}}
\newcommand{\nicolas}[1]{\mynote{Nicolas}{#1}}
\newcommand{\mdg}{\textit{Maven Dependency Graph}\@\xspace}
